A Design Recipe and Recipe-Based Errors for Regular Expressions

This article presents a novel framework to provide Formal Languages and Automata Theory students design support for the development of regular expressions. This framework includes a design recipe for regular expressions and a customized error messaging system. The error messaging system produces recipe-based errors that include the step of the design recipe not successfully completed. Furthermore, the error messages follow the established practices of being concise, succinct, jargon-free, and nonprescriptive. In addition, a shorthand syntax developed for writing unit tests is described. The in-class use of the design recipe is illustrated, two debugging sessions using the described system are discussed, and the implementation of the error messaging system is briefly sketched.

==> eptcsdata.tex <==
\providecommand{\firstpage}{25}
\providecommand{\publicationstatus}{Rose Bohrer (Ed.): Trends in Functional Programming\\ in Education (TFPiE).\\
EPTCS 424, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.424.2}{10.4204/EPTCS.424.2}}
\pdfoutput=1

